Hierarchically Disentangled Recurrent Network for Factorizing System Dynamics of Multi-scale Systems: An application on Hydrological Systems

We present a framework for modeling multi-scale processes, and study its performance in the context of streamflow forecasting in hydrology. Specifically, we propose a novel hierarchical recurrent neural architecture that factorizes the system dynamics at multiple temporal scales and captures their interactions. This framework consists of an inverse and a forward model. The inverse model is used to empirically resolve the system's temporal modes from data (physical model simulations, observed data, or a combination of them from the past), and these states are then used in the forward model to predict streamflow. Experiments on several catchments from the National Weather Service North Central River Forecast Center show that FHNN outperforms standard baselines, including physics-based models and transformer-based approaches. The model demonstrates particular effectiveness in catchments with low runoff ratios and colder climates. We further validate FHNN on the CAMELS (Catchment Attributes and MEteorology for Large-sample Studies), which is a widely used continental-scale hydrology benchmark dataset, confirming consistent performance improvements for 1-7 day streamflow forecasts across diverse hydrological conditions. Additionally, we show that FHNN can maintain accuracy even with limited training data through effective pre-training strategies and training global models.

==> 01_introduction_20250210.tex <==

\section{Introduction}
\label{sec:Introduction}

% \noindent\textcolor{blue}{\textit{physical systems have physical states that determine its response to external drivers}}

Physical systems, ranging from natural ecosystems to engineered structures, are characterized by complex interactions between internal states and external drivers. Response of such systems as a function of input drivers is governed by physical states that encapsulate their internal characteristics~\cite{ghosh2023entity}. For instance, in earth and environmental sciences, a catchment's streamflow response to meteorological drivers like precipitation and temperature is governed by complex physical processes specific to that basin~\cite{ghosh2022robust}. These processes involve factors such as snow-pack melting, and evapotranspiration in soil and plants. Figure~\ref{fig:related work}(a,b, and c) presents schematic representations of Forward models commonly used for understanding and predicting the behavior of these physical systems. 
% This model framework is widely applicable across fields like environmental sciences and engineering, enabling researchers to simulate complex systems and forecast their future states or behaviors~\cite{khandelwal2020physics}. Accurately capturing and incorporating these physical states is vital for a broad spectrum of applications, as they fundamentally determine how a system responds to external drivers. 
The forward model approach provides a structured way to represent these relationships, facilitating improved understanding and prediction of system dynamics in various scientific and engineering contexts.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{Images/forward and inverse.png}
%     \caption{\footnotesize \textit{Schematic representation of a Forward model illustrating the functional relationship $\mathcal{F}$ that maps the input $x^t$ along with a latent variable $z$ and the previous hidden state $h^{t-1}$ to the output $y^t$.}}
%     \label{fig:forward and inverse}
% \end{figure}

% \noindent\textcolor{blue}{\textit{PBM have been extensively used to model these}}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.85\linewidth]{Images/related work.png}
    \caption{\footnotesize \textit{Schematic of different modeling approaches for streamflow forecasting illustrating each approach's inputs, processes, and outputs. (a) Process-based Forward Models use weather forecasts to estimate catchment states and generate streamflow forecasts. (b) ML-based Forward Models (e.g., LSTM) directly use weather forecasts to predict streamflow forecasts. (c) ML-based Autoregressive Forward Models utilize weather forecasts and historical streamflow data for streamflow forecasting. (d) The proposed FHNN framework integrates an Inverse Model that generates catchment state representations from historical weather and streamflow data, which are then used alongside weather forecasts in a Forward Model to produce streamflow forecasts, capturing dynamics at multiple temporal scales (slow, medium, fast)}}
    \label{fig:related work}
\end{figure*}

Over the years, a number of physics-based models (PBMs) have been developed to represent different aspects of physical systems. For example, for streamflow modeling, the hydrological community makes extensive use of rainfall-runoff models~\cite{burnash1973generalizedsacsma} approximate the underlying bio-geophysical processes of the water cycle, shown in Figure~\ref{fig:related work}(a). Further, these models have been used in operational settings to forecast streamflow and water levels at NOAA’s National Weather Service (NWS). Such an operational setting requires a forecaster to assimilate real-time observations into the model, i.e., sequential data assimilation~\cite{bertino2003sequential}.

% Traditionally this is achieved through variational or Bayesian assimilation methods such as ensemble Kalman Filter (EnKF), that ingests observations in real-time to update the model states (for instance, catchment states in Figure~\ref{fig:related work}(a)). While Process-Based Models (PBMs) are widely adopted in the scientific community, they face challenges in fully capturing the complexity of environmental systems like hydrological catchments~\cite{kirchner2023instructive}. Many of the complex hydrological processes such as snow-pack depth, soil moisture distribution, and spatiotemporal variations in rainfall may not be replicated with high fidelity within the structure of a PBM, as they are necessarily approximation of the underlying phenomena~\cite{kirchner2023instructive}. Consequently, this impacts PBMs ability to accurately predict the physical quantities (fluxes) of interest, leading to unsatisfactory performance, especially in situations where insufficient observations are available to parametrize PBMs.

% \noindent\textcolor{blue}{\textit{ML specifically RNNs are being used nowadays. They build states.}}
ML models have shown tremendous success in computer vision and language modeling applications and are now increasingly being pursued in many scientific domains, including hydrology, where they have been shown to provide performance better than state-of-the-art process-based models in several settings ~\cite{feng2020enhancing,willard2022daily}. Specifically, time-aware deep learning techniques such as recurrent neural networks (RNNs) and Transformers have gained prominence as powerful tools for capturing temporal dependencies and building states~\cite{kratzert2019towards,yin2022rr}. Figure~\ref{fig:related work} (b) illustrates a diagrammatic representation of such ML based workflows. Transformers have been shown to be vastly superior to LSTM in language modeling tasks. In fact, Transformers have demonstrated remarkable success in time series forecasting across numerous domains, potentially due to their ability to capture long-range dependencies through self-attention mechanisms. \textcolor{red}{[Cite a couple of papers]}. Compared to LSTMs which process data sequentially, maintaining an evolving internal state, Transformers employ self-attention mechanisms to access all timesteps simultaneously. However, their superiority is less clear for modeling environmental science phenomena, where the objective is to model a variable of interest over time, in response to drivers (e.g., weather) and local characteristics \textcolor{red}{[take Praveen Figure?]}. Note that in language modeling,  current states depend primarily on direct  e.g.historical relationships, whereas in environmental systems, the response is driven by cumulative path-dependent effects (memory) \textcolor{red}{like xxx, yyy [cite more papers]}.  For example, In hydrology, current streamflow depends not only on recent precipitation but on the sequential evolution of soil moisture, and groundwater levels. Similar path dependencies appear in Many other environmental applications; e.g. soil biochemistry, where nutrient cycles depend on previous microbial activity and organic matter decomposition follows sequential patterns.

Transformers also tend to be data hungry. The reason is that the attention mechanisms in transformers are approximating the evolution of states in a path-dependent system through multi-headed attention over all historical timesteps and are essentially memory machines ~\cite{mahdavi2023memorization,geva2020transformer,carlini2022quantifying}. The limited availability of training data further compounds the challenges for Transformers can perform poorly when all examples of such paths are not present in the training data. Hydrological records tend to be sparse. For many regions of the world, stream-flow data exists for only a few years. Even  in data rich regions such as North America, such data is available only for a few decades, that too only  for large basins. Such constraints tend to favor LSTM's inductive bias, whose architecture explicitly models sequential state evolution through internal memory states. Indeed this is confirmed by a number of comparative studies between transformer and LSTM based models.  Indeed, for hydrological modeling, a number of papers have shown that Transformer based models underperform LSTM based models \textcolor{red}{~\cite{}(cite …..)}. 

Current machine learning models, including RNNs, do not represent states explicitly at multiple temporal scales or model their interactions. Environmental systems often feature phenomena that evolve at different time scales, from rapid fluctuations to slowly changing trends. For instance, the impact of the location of rainfall on runoff is evident at hourly/daily and seasonal scales~\cite{zhou2021impacts}. The soil moisture state of a catchment is built up at a weekly scale and thus needs a longer window of information. On the other hand, snow-pack is accumulated at a monthly scale and thus takes longer to impact a catchment's runoff (snow accumulation in December impacts stage and discharge in April)~\cite{dingman2015physical}. Thus, standard RNN's inability to explicitly model such states that are evolving and interacting at different scales, hinders their effectiveness in capturing the full behavior spectrum of complex physical systems with interdependent multi-scale dynamics


In an operational setting, two main data assimilation approaches are used for integrating new data into RNN-based ML models. The first applies Kalman filter variants to the RNN's recurrent structure, optimizing a loss function, typically a regularized mean squared error during test time or deployment \cite{zwart2023near,nearing2021data}. The second, simpler and more computationally efficient method employs an auto-regressive RNN, where the previous timestep's actual output is used as an additional input alongside other weather drivers \cite{feng2020enhancing} (see Figure~\ref{fig:related work}c).


% \noindent\textcolor{blue}{\textit{we propose a model that build states at different temporal scales}}

In this paper, we propose a novel factorized hierarchical neural network (FHNN) architecture (Figure~\ref{fig:related work}d) that factorizes the system dynamics at multiple temporal scales and captures their interactions. This framework consists of an inverse and a forward model. The inverse model is used to empirically resolve the system's temporal modes from data (physical model simulations, observed data, or a combination of them from the past), and these states are then used in the forward model to predict streamflow. In a hydrological system, these modes can represent different processes, evolving at different temporal scales (e.g., slow: groundwater recharge vs. fast: surface runoff due to extreme rainfall). 

Two key advantages of our approach are: 1) it can model processes that are evolving and interacting at multiple scales, and 2) Once trained, it can incorporate new observations into the model's context (internal state) without expensive optimization approaches  (e.g., Ensemble Kalman Filtering) that are traditionally used in physical sciences for data assimilation. Experiments with several river catchments from the National Weather Service (NWS) North Central River Forecast Center region show the efficacy of this ML-based data assimilation framework compared to standard baselines, especially for basins that have a long history of observations. To handle basins with a short observation history, we present two orthogonal strategies for training our FHNN framework: (a) using simulation data from imperfect simulations and (b) using observation data from multiple basins to build a global model.  We show that both of these strategies (that can be used individually or together) are highly effective in mitigating the lack of training data. The improvement in forecast accuracy is particularly noteworthy for basins where local models perform poorly because of data sparsity. While demonstrated in the context of hydrological streamflow modeling, our proposed framework's effectiveness in modeling multi-scale processes makes it useful for a wide variety of science and engineering applications. Our main contributions are listed below:

$\bullet$ We introduce FHNN, a novel architecture that models multi-scale dynamics by factorizing system states at different temporal scales.

$\bullet$ We demonstrate two effective strategies for mitigating data sparsity in hydrological modeling: 1) pre-training FHNN on simulated NWS SAC-SMA model (a PBM) outputs and 2) developing a global model trained across multiple basins. Both approaches significantly improve FHNN's performance with limited observations.

$\bullet$ FHNN demonstrates superior performance over state-of-the-art ML approaches across multiple river basins in the NWS-RFC operational region.

$\bullet$ We evaluate FHNN on the CAMELS dataset, a continental-scale hydrology benchmark, showing consistent outperformance over baseline models for short-term (1-day) to medium-term (7-day) streamflow forecasts.

$\bullet$ We provide interpretable visualizations of the learned multi-scale states, offering insights into the model's representation of hydrological processes at different temporal scales.

==> 03_preliminariesRelatedWork_20250210.tex <==
\section{Preliminaries and Related Works}
\label{sec:Preliminaries and Related Works}
\noindent\textbf{Predictive Modeling for Dynamical Systems:} ML models have been extensively used by the scientific community as emulators of physics-based models~\cite{lall2014debates}. A significant advantage of pure ML is its ability to be entirely data-driven, bypassing the need for causal structures derived from domain knowledge, which can often be incomplete. In hydrology, Standard RNNs and their variants Long Short-Term Memory (LSTM) networks have been widely used to predict variables like water temperature~\cite{zwart2023near,willard2022daily} and water level~\cite{bowes2019forecasting}. When modeling driver-response relationships, using an RNN equipped with LSTM cells or similar LSTM variants is quite intuitive, as shown in Figure~\ref{fig:related work} (b). LSTM-based models have achieved state-of-the-art performance in streamflow modeling~\cite{kratzert2019towards} and flood-forecasting~\cite{nearing2024global,yin2021rainfall}. LSTM models trained on multi-basin data capture diverse rainfall-runoff responses, enhancing predictions by leveraging knowledge from large datasets.

Recently, Transformers have gained prominence as powerful tools for capturing temporal dependencies and building states~\cite{kratzert2019towards,yin2022rr}. Transformers have been shown to be vastly superior to LSTM in language modeling tasks. In fact, Transformers have demonstrated remarkable success in time series forecasting across numerous domains, potentially due to their ability to capture long-range dependencies through self-attention mechanisms. \cite{tayal2024exotst,YuqietalPatchTST, liu2023itransformer, zhang2023crossformer}. Compared to LSTMs which process data sequentially, maintaining an evolving internal state, Transformers employ self-attention mechanisms to access all timesteps simultaneously. However, their superiority is less clear for modeling environmental science phenomena, where the objective is to model a variable of interest over time, in response to drivers (e.g., weather) and local characteristics. Note that in language modeling,  current states depend primarily on direct  e.g.historical relationships, whereas in environmental systems, the response is driven by cumulative path-dependent effects (memory) ~\cite{boehrer2008stratification,jia2017state}.  For example, In hydrology, current streamflow depends not only on recent precipitation but on the sequential evolution of soil moisture, and groundwater levels. Similar path dependencies appear in many other environmental applications; e.g. soil biochemistry, where nutrient cycles depend on previous microbial activity and organic matter decomposition follows sequential patterns.

Transformers also tend to be data hungry. The reason is that the attention mechanisms in transformers are approximating the evolution of states in a path-dependent system through multi-headed attention over all historical timesteps and are essentially memory machines ~\cite{mahdavi2023memorization,geva2020transformer,carlini2022quantifying}. The limited availability of training data further compounds the challenges for Transformers can perform poorly when all examples of such paths are not present in the training data. Hydrological records tend to be sparse. For many regions of the world, stream-flow data exists for only a few years. Even in data rich regions such as North America, such data is available only for a few decades, that too only for large basins. Such constraints tend to favor LSTM's inductive bias, whose architecture explicitly models sequential state evolution through internal memory states. Indeed this is confirmed by a number of comparative studies between transformer and LSTM based models.  Indeed, for hydrological modeling, a number of papers have shown that Transformer based models underperform LSTM based models ~\cite{liu2024probing}.

\noindent\textbf{Forecasting for Dynamical Systems:} The standard LSTM model cannot ingest near-real-time response data and perform data assimilation. Thus, a simple extension to the standard LSTM is to provide lagged response data as input for the model. Several studies~\cite{feng2020enhancing,moshe2020hydronets} have shown that autoregression (AR) improves streamflow predictions from LSTMs. Figure~\ref{fig:related work} (c) shows the diagrammatic representation of the PBM.

\begin{figure*}[t]
    \begin{subfigure}{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Images/hdlvm.png}
        \caption{}
        \label{fig:Graph}
    \end{subfigure}
    \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Images/model.png}
        \caption{}
        \label{fig:Architecture}
    \end{subfigure}
    \caption{\footnotesize(a) \textit{Graphical model representation of FHNN for time series data. The model illustrates the relationships between latent variables ($z_0$ to $z_l$), observed variables ($x$ and $y$), and model parameters ($\phi$ and $\theta$). It shows the generative process ($p_{\theta}(\boldsymbol{Y^t}|\boldsymbol{z}, \boldsymbol{X^t})$) and the inference process ($q_{\phi}(\boldsymbol{z}|\boldsymbol{X^{t-1}}, \boldsymbol{Y^{t-1}}$), depicting how past observations influence the current latent state and how the current latent state and inputs generate the output. This structure enables FHNN to capture multi-scale temporal dependencies and generate predictions.}, (b) \textit{Architecture of FHNN for streamflow prediction. The model processes historical weather and streamflow data at three different timescales (fast, medium, and slow) using parallel BiLSTM layers, capturing temporal dependencies at various resolutions. The final hidden states from each timescale ($h_f$, $h_m$, $h_s$) are combined with forecasted weather data to generate streamflow predictions for future time steps. This design allows the model to integrate both short-term fluctuations and long-term trends in the input data for more accurate streamflow forecasting.}}
\end{figure*}

\noindent\textbf{Knowledge-guided Machine Learning:} Knowledge-guided Machine Learning~\cite{willard2022integrating} demonstrates the benefits of integrating domain knowledge to enhance ML models. One effective approach is the knowledge-guided architecture, which incorporates known hierarchical structures among processes when designing an ML model~\cite{khandelwal2020physics}. These models outperform direct driver-to-response mappings by embedding physical principles into the network architecture and modifying existing components to align with assumptions about interacting physical processes/states. Recently, learnable, differentiable process-based models~\cite{feng2023suitability} with embedded neural networks have been shown to achieve predictive performance comparable to LSTM models. Despite their promise, these models' rigid architectural design poses challenges similar to those of traditional process-based models. Our framework addresses the need to model the internal states of a dynamical system while maintaining the flexibility to allow the model to discover processes not captured in existing domain knowledge.

